Dualities and non-Abelian mechanics

Dualities are mathematical mappings that reveal unexpected links between apparently unrelated systems or quantities in virtually every branch of physics. Systems that are mapped onto themselves by a duality transformation are called self-dual and they often exhibit remarkable properties, as exemplified by an Ising magnet at the critical point. In this Letter, we unveil the role of dualities in mechanics by considering a family of so-called twisted Kagome lattices. These are reconfigurable structures that can change shape thanks to a collapse mechanism easily illustrated using LEGO. Surprisingly, pairs of distinct configurations along the mechanism exhibit the same spectrum of vibrational modes. We show that this puzzling property arises from the existence of a duality transformation between pairs of configurations on either side of a mechanical critical point. This critical point corresponds to a self-dual structure whose vibrational spectrum is two-fold degenerate over the entire Brillouin zone. The two-fold degeneracy originates from a general version of Kramers theorem that applies to classical waves in addition to quantum systems with fermionic time-reversal invariance. We show that the vibrational modes of the self-dual mechanical systems exhibit non-Abelian geometric phases that affect the semi-classical propagation of wave packets. Our results apply to linear systems beyond mechanics and illustrate how dualities can be harnessed to design metamaterials with anomalous symmetries and non-commuting responses.

==> crystallographic_notations.tex <==
\RequirePackage{expl3,xparse,l3regex}
\ExplSyntaxOn
% Hermann-Mauguin symbols for space and point groups.
% The command \hm transforms the usual text version of Hermann-Mauguin symbols into a LaTeX version. 
% Explicitly, 
% 1) -x is replaced by \overline{x}
% 2) x_y is indeed a subscript
% where x and y are single characters.
% Additionally, text characters [a-zA-Z] are put into text mode (x replaced by \text{x})
% and the entire symbol is put in math mode (through \ensuremath).
% Example: \hm{I4_132} outputs something like I4₁32
% Example: \hm{Ia-3d} outputs something like Ia3̅d
% Example: \def\mySpaceGroup{P-42_1c} \hm{\mySpaceGroup} outputs P4̅2₁c
\NewDocumentCommand{\hm}{m}
{
    \tl_set:Nx \l_hm_contents {\ensuremath{#1}}
    \regex_replace_all:nnN { -(.) } { \c{overline}\cB\{ \1 \cE\} } \l_hm_contents
    \regex_replace_all:nnN { (.)\_(.) } { \1\c{c_math_subscript_token}\2 } \l_hm_contents
    \regex_replace_all:nnN { ([a-zA-Z]+) } { \c{text}\cB\{ \1 \cE\} } \l_hm_contents
    \tl_use:N \l_hm_contents
}

% Schoenflies symbols for point groups.
% The command \sch transforms a textual representation of Schoenflies symbols into a LaTeX version.
% Symmetry operations are not supported for the moment, as understanding both symbols for point groups and
% the corresponding symmetry operations would require an actual parsing instead of a band-aid regex implementation.
%
% The convention for typesetting such symbols are from the article
% Notations and conventions in molecular spectroscopy: Part 2. Symmetry notation (IUPAC Recommendations 1997)
% C. J. H. Schutte / J. E. Bertie / P. R. Bunker / J. T. Hougen / I. M. Mills / J. K. G. Watson / B. P. Winnewisser
% Pure and Applied Chemistry. Volume 69, Issue 8, Pages 1641–1650, ISSN (Online) 1365-3075, ISSN (Print) 0033-4545
% DOI: https://doi.org/10.1351/pac199769081641, January 2009
% which is nicely summarized in http://chemistry.stackexchange.com/a/32939
\NewDocumentCommand{\sch}{m}
{
    \tl_set:Nx \l_sch_contents {#1}
    \regex_replace_all:nnN { \_ }{} \l_sch_contents % remove the subscript character _ as we take care of that
%    \regex_replace_all:nnN {\c{infty}}{\c{text}\cB\{\c{c_math_toggle_token}\c{infty}\c{c_math_toggle_token}\cE\}} \l_sch_contents % useless, was used to ensure that the \infty was working
    \regex_replace_all:nnN { (.)(.*) } { \1\c{c_math_subscript_token}\cB\{\2\cE\} } \l_sch_contents % all except the first character is in subscript
    \regex_replace_all:nnN { (d|h|v|s) }{ \c{text}\cB\{\1\cE\} }  \l_sch_contents % replace d,h,v,s with their upright version (all other letters are left in italic as they are not part of the Schoenflies symbol, and are therefore expected to be a variable name
    \regex_replace_all:nnN { \cS\  }{} \l_sch_contents % remove spaces
    \tl_set:Nn \l_sch_result {\ensuremath{\l_sch_contents}} % ensure that everything is in math mode
    \tl_use:N \l_sch_result
}

% Irreducible representation symbols. 
% The command \irrep transforms a text representation of an irreducible representation into a LaTeX version.
% Explicitly, all letters are set upright, and everything but the first cahracter is in subscript.
% This is not ideal, but a good first start.
\NewDocumentCommand{\irrep}{m}
{
    \tl_set:Nx \l_sch_contents {#1}
    \regex_replace_all:nnN { \_ }{} \l_sch_contents % remove the subscript character _ as we take care of that
    \regex_replace_all:nnN { (.)(.*) } { \1\c{c_math_subscript_token}\cB\{\2\cE\} } \l_sch_contents % all except the first character is in subscript
    \regex_replace_all:nnN { ([a-zA-Z]) }{ \c{text}\cB\{\1\cE\} }  \l_sch_contents % all letters are upright
    \regex_replace_all:nnN { \cS\  }{} \l_sch_contents % remove spaces
    \tl_set:Nn \l_sch_result {\ensuremath{\l_sch_contents}} % ensure that everything is in math mode
    \tl_use:N \l_sch_result
}
\ExplSyntaxOff

% See http://www.iucr.org/resources/symmetry-font
% and https://ctan.org/pkg/cryst
\DeclareFontFamily{U}{crystallographicSymbol}{\hyphenchar\font=-1}
\DeclareFontShape{U}{crystallographicSymbol}{m}{n}{ <-> cryst}{}
\newcommand{\crystallographicSymbol}[1]{{\usefont{U}{crystallographicSymbol}{m}{n} \symbol{#1}}}
